UniMoD: Efficient Unified Multimodal Transformers with Mixture-of-Depths

Unified multimodal transformers, which handle both generation and understanding tasks within a shared parameter space, have received increasing attention in recent research. Although various unified transformers have been proposed, training these models is costly due to redundant tokens and heavy attention computation. In the past, studies on large language models have demonstrated that token pruning methods, such as Mixture of Depths (MoD), can significantly improve computational efficiency. MoD employs a router to select the most important ones for processing within a transformer layer. However, directly applying MoD-based token pruning to unified transformers will result in suboptimal performance because different tasks exhibit varying levels of token redundancy. In our work, we analyze the unified transformers by (1) examining attention weight patterns, (2) evaluating the layer importance and token redundancy, and (3) analyzing task interactions. Our findings reveal that token redundancy is primarily influenced by different tasks and layers. Building on these findings, we introduce UniMoD, a task-aware token pruning method that employs a separate router for each task to determine which tokens should be pruned. We apply our method to Show-o and Emu3, reducing training FLOPs by approximately 15% in Show-o and 40% in Emu3, while maintaining or improving performance on several benchmarks. Code will be released at https://github.com/showlab/UniMoD.

==> tables/table_baselines.tex <==


\definecolor{myyellow}{rgb}{1,1, 0.6}
\definecolor{myorange}{rgb}{1, 0.8, 0.6}
\definecolor{myred}{rgb}{1, 0.6, 0.6}
\definecolor{mygray}{gray}{0.6} 

\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{llccccccccc}
        \toprule

             Method & Params & TFLOPS$\downarrow$ & Training Cost$\downarrow$  & POPE$\uparrow$ & MME$\uparrow$ & VQAv2$_{\text{(test)}}$$\uparrow$ & GQA$\uparrow$ & MMMU$\uparrow$ &GenEval$\uparrow$  \\
    	\midrule
             % \textcolor{mygray}{NExT-GPT}~\cite{wu2023next} & \textcolor{mygray}{13B} &  \textcolor{mygray}{-} &  \textcolor{mygray}{-} &  \textcolor{mygray}{84.5}  &  \textcolor{mygray}{-} &  \textcolor{mygray}{-} & \textcolor{mygray}{-}&\textcolor{mygray}{-}&\textcolor{mygray}{-}\\
             
             % \textcolor{mygray}{SEED-X}~\cite{seed-x} & \textcolor{mygray}{17B} & \textcolor{mygray}{-} & \textcolor{mygray}{-} & \textcolor{mygray}{84.2} & \textcolor{mygray}{1435.7} & \textcolor{mygray}{52.3} & \textcolor{mygray}{47.9} & \textcolor{mygray}{35.6} & \textcolor{mygray}{0.49}\\
             
             % \textcolor{mygray}{VILA-U~\cite{vila-u}} &  \textcolor{mygray}{7B}& \textcolor{mygray}{-} & \textcolor{mygray}{-}&  \textcolor{mygray}{85.8} & \textcolor{mygray}{1401.8} & \textcolor{mygray}{-} & \textcolor{mygray}{60.8} & \textcolor{mygray}{31.6} & \textcolor{mygray}{-}\\
             
             % \textcolor{mygray}{Emu3~\cite{emu3}} &   \textcolor{mygray}{8B} & \textcolor{mygray}{-}& \textcolor{mygray}{-}&  \textcolor{mygray}{85.2} &  \textcolor{mygray}{-} &  \textcolor{mygray}{-}  &  \textcolor{mygray}{60.3} & \textcolor{mygray}{-} &  \textcolor{mygray}{0.66} \\
             
              % \textcolor{mygray}{Chameleon}~\cite{team2024chameleon} &   \textcolor{mygray}{34B} & \textcolor{mygray}{-} & \textcolor{mygray}{-} &  \textcolor{mygray}{74.7}  &  \textcolor{mygray}{-} &  \textcolor{mygray}{-}& \textcolor{mygray}{-} & \textcolor{mygray}{-}& \textcolor{mygray}{0.39}\\

             % \textbf{Full Computation} & 1.3B & 30.94 & 32G & \underline{77.94} & \underline{1032} & \textbf{62.39} & \textbf{52.54} & \textbf{27.44} & \textbf{0.64}\\  
             % \textbf{LayerSkip} &1.3B  & \textbf{15.65}& \textbf{22G}& 73.69 & 796 & 51.25 & 43.55 &25.67 &  0.37\\      
             % \textbf{EarlyExit} & 1.3B & \textbf{15.65} & \textbf{22G}& 77.47 & 968  &  57.26 & 48.6 & 26.11 & \underline{0.42} \\  
             
             % \textbf{\method{}} & 1.3B & \underline{23.30}& \underline{27G} & \textbf{78.07} & \textbf{1045} & \underline{61.51} &  \underline{51.80} & \underline{27.22}  & \textbf{0.64}\\  

            \textbf{Full Computation} & 1.3B & 30.94 & 32G & \underline{77.94} & \underline{1032} & \textbf{62.39} & \textbf{52.54} & \textbf{27.44} & \textbf{0.64}\\  
             \textbf{LayerSkip} &1.3B  & \textbf{15.65}& \textbf{22G}& 73.69 & 796 & 51.25 & 43.55 &25.67 &  0.37\\      
             \textbf{EarlyExit} & 1.3B & \textbf{15.65} & \textbf{22G}& 77.47 & 968  &  57.26 & 48.6 & 26.11 & \underline{0.42} \\  
             
             \textbf{\method{}(Show-o)} & 1.3B & \underline{23.30}& \underline{26G} & \textbf{78.07} & \textbf{1045} & \underline{61.51} &  \underline{51.80} & \underline{27.22}  & \textbf{0.64}\\   
            
        \bottomrule

\end{tabular}
}
% \caption{Comparison with Baseline Methods. We evaluate our approach against EarlyExit, LayerSkip, and Full Computation baselines on both Multi-Modal Understanding (mmu) and Text-to-Image (t2i) benchmarks. Additionally, we compare TFLOPs and training memory usage. Our method achieves the best balance between performance and efficiency across all metrics. We color code each cell, highlighting \textbf{\textbf{the best results}} and \underline{\textbf{the second-best results}.}}

\caption{Comparison with Baseline Methods. We evaluate our approach against EarlyExit, LayerSkip, and Full Computation baselines on both Multi-Modal Understanding (MMU) and Text-to-Image (T2I) benchmarks. Additionally, we compare TFLOPs and training memory usage. Our method achieves the best balance between performance and efficiency across all metrics. We color code each cell, highlighting \textbf{the best results} and \underline{the second-best results}.}
\label{tab:table_baselines}
\end{table*}


==> tables/table_baselines2.tex <==


\definecolor{myyellow}{rgb}{1,1, 0.6}
\definecolor{myorange}{rgb}{1, 0.8, 0.6}
\definecolor{myred}{rgb}{1, 0.6, 0.6}
\definecolor{mygray}{gray}{0.6} 

\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{ 
\begin{tabular}{llccccccccc}
        \toprule

             Model & Method & Params & TFLOPS$\downarrow$ & Training Cost$\downarrow$  & POPE$\uparrow$ & MME$\uparrow$ & VQAv2$_{\text{(test)}}$$\uparrow$ & GQA$\uparrow$ & MMMU$\uparrow$ &GenEval$\uparrow$  \\
    	\midrule
             \multirow{4}{*}{Show-o}&
            Full Computation & 1.3B & 30.94 & 32G & \underline{77.94} & \underline{1032} & \textbf{62.39} & \textbf{52.54} & \textbf{27.44} & \textbf{0.64}\\  
            
             & LayerSkip &1.3B  & \textbf{15.65}& \textbf{22G}& 73.69 & 796 & 51.25 & 43.55 &25.67 &  0.37\\ 
             
             & EarlyExit & 1.3B & \textbf{15.65} & \textbf{22G}& 77.47 & 968  &  57.26 & 48.6 & 26.11 & \underline{0.42} \\  
             
             & \method{} & 1.3B & \underline{23.30}& \underline{27G} & \textbf{78.07} & \textbf{1045} & \underline{61.51} &  \underline{51.80} & \underline{27.22}  & \textbf{0.64}\\   
            
        \bottomrule

\end{tabular}
}
\caption{Comparison with Baseline Methods. We evaluate our approach against EarlyExit, LayerSkip, and Full Computation baselines on both Multi-Modal Understanding (MMU) and Text-to-Image (T2I) benchmarks. Additionally, we compare TFLOPs and training memory usage. Our method achieves the best balance between performance and efficiency across all metrics. We color code each cell, highlighting \textbf{the best results} and \underline{the second-best results}.}
\label{tab:table_baselines2}
\end{table*}


==> tables/table_baselines3.tex <==



% \begin{table}[t]
% \centering
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{llcccccc}
%         \toprule

%               Method & POPE$\uparrow$ & MME$\uparrow$ & VQAv2$_{\text{(test)}}$$\uparrow$ & GQA$\uparrow$ & MMMU$\uparrow$ &GenEval$\uparrow$  \\
%     	\midrule
           
%             Show-o & \underline{77.94} & \underline{1032} & \textbf{62.39} & \textbf{52.54} & \textbf{27.44} & \textbf{0.64}\\  
            
%              LayerSkip  & 73.69 & 796 & 51.25 & 43.55 &25.67 &  0.37\\ 
             
%               EarlyExit  & 77.47 & 968  &  57.26 & 48.6 & 26.11 & \underline{0.42} \\  
             
%               \method{}   & \textbf{78.07} & \textbf{1045} & \underline{61.51} &  \underline{51.80} & \underline{27.22}  & \textbf{0.64}\\   
            
%         \bottomrule

% \end{tabular}
% }
% \caption{Comparison with Baseline Methods. We evaluate our approach against EarlyExit, LayerSkip, and Full Computation baselines on both Multi-Modal Understanding (MMU) and Text-to-Image (T2I) benchmarks. We color code each cell, highlighting \textbf{the best results} and \underline{the second-best results}.}
% \vspace{-10pt}
% \label{tab:table_baselines2}
% \end{table}




% \begin{table*}[t]
% \centering
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{llccccccccc}
%         \toprule

%              Model & Method & Params & TFLOPS$\downarrow$ & POPE$\uparrow$ & MME$\uparrow$ & VQAv2$_{\text{(test)}}$$\uparrow$ & GQA$\uparrow$ & MMMU$\uparrow$ &GenEval$\uparrow$  \\
%     	\midrule
%              \multirow{4}{*}{Show-o}&
%             Full Computation & 1.4B & 30.94 & \underline{77.94} & \underline{1032} & \textbf{62.39} & \textbf{52.54} & \textbf{27.44} & \textbf{0.64}\\  
            
%              & LayerSkip &1.4B  & \textbf{15.65}& 73.69 & 796 & 51.25 & 43.55 &25.67 &  0.37\\ 
             
%              & EarlyExit & 1.4B & \textbf{15.65} & 77.47 & 968  &  57.26 & 48.6 & 26.11 & \underline{0.42} \\  
             
%              & \method{} & 1.4B & \underline{23.30} & \textbf{78.07} & \textbf{1045} & \underline{61.51} &  \underline{51.80} & \underline{27.22}  & \textbf{0.64}\\   
            
%         \bottomrule

% \end{tabular}
% }
% \caption{Comparison with Baseline Methods. We evaluate our approach against EarlyExit, LayerSkip, and Full Computation baselines on both Multi-Modal Understanding (MMU) and Text-to-Image (T2I) benchmarks. Additionally, we compare TFLOPs and training memory usage. Our method achieves the best balance between performance and efficiency across all metrics. We color code each cell, highlighting \textbf{the best results} and \underline{the second-best results}.}
% \label{tab:table_baselines2}
% \end{table*}




% \begin{wraptable}{r}{0.6\textwidth}
% \usepackage{wrapfig}

% \definecolor{lightblue}{RGB}{235, 245, 255}

\begin{table}
\centering

\resizebox{1\linewidth}{!}{

\centering
\setlength{\tabcolsep}{1.8pt}

% %
\begin{tabular}{l|ccccccc}
% \begin{tabular}{l||ccccc||ccccc}
\toprule

\multicolumn{1}{l|}{}
&\multicolumn{1}{c}{ TFLOPS$\downarrow$ }
&\multicolumn{1}{c}{ MME$\uparrow$ }
&\multicolumn{1}{c}{ GQA$\uparrow$ }
&\multicolumn{1}{c}{ POPE$\uparrow$ }
&\multicolumn{1}{c}{ MMMU$\uparrow$ }
% &\multicolumn{1}{c}{ VQAv2{\text{(test)}}$\uparrow$ }
&\multicolumn{1}{c}{ VQAv2$\uparrow$ }
&\multicolumn{1}{c}{ GenEval$\uparrow$ }



  \\
  \midrule
  Full
  &$51.1$
  &$1056$
  &$56.29$
  &$79.80$ 
  &$25.78$
  &$68.34$ 
  &$0.62$

  \\LayerSkip
  &$25.6$
  &$828$
  &$45.63$
  &$74.19$ 
  &$27.22$
  &$53.92$ 
  &$0.29$

   \\EarlyExit
  &$25.6$
  &$947$
  &$51.07$
  &$79.48$ 
  &$24.11$
  &$60.42$ 
  &$0.26$


  \\
  \rowcolor{lightblue} 
  \method{}
  &$43.3$
  &$1094$
  &$54.49$
  &$80.28$ 
  &$25.67$
  &$66.24$ 
  &$0.61$



\\ \bottomrule


\end{tabular}

}

\caption{Comparison of UniMoD with baseline methods—EarlyExit, LayerSkip, and Full Computation—in the Show-o model across Multi-Modal Understanding (MMU) and Text-to-Image (T2I) benchmarks.}

\label{tab:table_baselines3}
\vspace{-10pt}
\end{table}
% \end{wraptable}
% 


% \begin{table*}
% \centering

% \resizebox{1\linewidth}{!}{

% \centering
% \setlength{\tabcolsep}{1.8pt}

% %
% \begin{tabular}{l|cccccccc}
% % \begin{tabular}{l||ccccc||ccccc}
% \toprule

% \multicolumn{1}{l|}{}
% &\multicolumn{1}{c}{ Params$\downarrow$ }
% &\multicolumn{1}{c}{ TFLOPS$\downarrow$ }
% &\multicolumn{1}{c}{ MME$\uparrow$ }
% &\multicolumn{1}{c}{ GQA$\uparrow$ }
% &\multicolumn{1}{c}{ POPE$\uparrow$ }
% &\multicolumn{1}{c}{ MMMU$\uparrow$ }
% &\multicolumn{1}{c}{ VQAv2{\text{(test)}}$\uparrow$ }
% % &\multicolumn{1}{c}{ VQAv2$\uparrow$ }
% &\multicolumn{1}{c}{ GenEval$\uparrow$ }



%   \\
%   \midrule
%   Full Computation
%   &$51.1$
%   &$1056$
%   &$56.29$
%   &$79.80$ 
%   &$25.78$
%   &$68.34$ 
%   &$0.62$

%   \\LayerSkip
%   &$25.6$
%   &$828$
%   &$45.63$
%   &$74.19$ 
%   &$27.22$
%   &$53.92$ 
%   &$0.29$

%    \\EarlyExit
%   &$25.6$
%   &$947$
%   &$51.07$
%   &$79.48$ 
%   &$24.11$
%   &$60.42$ 
%   &$0.26$


%   \\
%   \rowcolor{lightblue} 
%   \method{}
%   &$43.3$
%   &$1094$
%   &$54.49$
%   &$80.28$ 
%   &$25.67$
%   &$66.24$ 
%   &$0.61$



% \\ \bottomrule


% \end{tabular}

% }

% \caption{Comparison of UniMoD with baseline methods—EarlyExit, LayerSkip, and Full Model—in the Show-o model across Multi-Modal Understanding (MMU) and Text-to-Image (T2I) benchmarks.}

% \label{tab:table_baselines3}
% \vspace{-10pt}
% \end{table*}

==> tables/table_comparsion_new_data.tex <==


% \begin{wraptable}{r}{0.3\textwidth}
% \usepackage{wrapfig}
\begin{table}
\centering

\resizebox{1\linewidth}{!}{

\centering
\setlength{\tabcolsep}{1.8pt}

%
\begin{tabular}{lcccccc}
% \begin{tabular}{l||ccccc||ccccc}
\toprule

\multicolumn{1}{l}{Benchmark}
&\multicolumn{1}{c}{ MME$\uparrow$ }
&\multicolumn{1}{c}{ GQA$\uparrow$ }
&\multicolumn{1}{c}{ POPE$\uparrow$ }
&\multicolumn{1}{c}{ MMMU$\uparrow$ }
&\multicolumn{1}{c}{ VQAv2{\text{(test)}}$\uparrow$ }
&\multicolumn{1}{c}{ GenEval$\uparrow$ }


  \\
   \midrule
  Show-o*
  &$1032$
  &$52.54$
  &$77.94$ 
  &$27.44$
  &$62.39$ 
  &$0.64$



\\ \bottomrule


\end{tabular}

}
\caption{Show-o represent the original Show-o model. Show-o* represents the model with new data. We both use 256 resolution images to train and test.}
\label{tab:comparison_showo}

\vspace{-10pt}
\end{table}
% \end{wraptable}



==> tables/table_emu3.tex <==

% \begin{table*}[t]
% \centering
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{llcccccccc|c|c}
%         \toprule
%     	Model & Method & TFLOPS$\downarrow$ & Training Cost$\downarrow$ & Single Obj. & Two Obj. & Counting  & Colors &  Position & Color Attri. & Overall GenEval$\uparrow$  & Flickr30k$\uparrow$\\
%         \midrule
%             \multirow{3}{*}{Emu3}
%             & Original Model & 88.986  &3.19s/iter &0.89 &0.46 &0.17 &0.66 &0.10 &0.25 &0.423  & 5.24\\
%             & Full Computation & 88.986 &3.19s/iter  &0.90 & 0.56 & 0.24 & 0.72 & 0.13 & 0.18&  \underline{0.456} & \underline{17.6} \\
%              & \method{} & 53.489& 1.97s/iter &0.96 & 0.60 & 0.26 & 0.73 & 0.15 & 0.24 & \textbf{0.488} & \textbf{18.2} \\
%         \bottomrule

% \end{tabular}
% }

% % \caption{MoD for PixArt. We find ARank-based MoD achieves the closest result with the full computation model. We color code each cell, highlighting \textbf{\textbf{the best results}} and \underline{\textbf{the second-best results}}}
% \caption{MoD for EMU3. Our method outperforms the full computation model in both generation and captioning tasks. Each cell is bolded to highlight \textbf{the best results} and \underline{the second-best results}.}

% \label{tab:table_emu3}
% \end{table*}




% \begin{wraptable}{r}{0.6\textwidth}
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{llcccccccc|c|c}
%         \toprule
%     	Model & Method  & TFLOPS$\downarrow$ & Training Cost$\downarrow$ & GenEval$\uparrow$  & Flickr30k$\uparrow$\\
%         \midrule
%             \multirow{3}{*}{Emu3}
%             & Original Model & 88.986  &72.5G  &0.423  & 5.24\\
%             & Full Computation & 88.986 &72.5G  &  \underline{0.456} & \underline{17.6} \\
%              & \method{}  &53.489& 67.5G & \textbf{0.488} & \textbf{18.2} \\
%         \bottomrule
% \end{tabular}
% }
% \caption{UniMoD for Emu3. Our method outperforms the full computation model in both generation and captioning tasks. Each cell is bolded to highlight \textbf{the best results} and \underline{the second-best results}.}
% \vspace{-10pt}

% \label{tab:table_emu3}
% \end{table}


% \definecolor{mygray}{gray}{0.6} 
% \definecolor{lightblue}{RGB}{235, 245, 255}
% \begin{table}
% \centering
% \resizebox{\linewidth}{!}{ 
% \begin{tabular}{llccccccc|c|c}
%         \toprule
%     	Model & Method  & TFLOPS$\downarrow$ & GenEval$\uparrow$  & Flickr30k$\uparrow$\\
%         \midrule
%             \multirow{3}{*}{Emu3}
            
%             & \textcolor{mygray}{Base Model} &  \textcolor{mygray}{88.986}    & \textcolor{mygray}{0.423}  &  \textcolor{mygray}{5.24}\\
%             & Full Computation & 88.986   &  0.456 & 17.6 \\
%             \rowcolor{lightblue} 
%              & \method{}  &53.489 & 0.488 & 18.2 \\
%         \bottomrule
% \end{tabular}
% }
% \caption{UniMoD for Emu3. Our method outperforms the full computation model in both generation and captioning tasks. Each cell is bolded to highlight \textbf{the best results} and \underline{the second-best results}.}
% \vspace{-10pt}

% \label{tab:table_emu3}
% \end{table}


% \definecolor{mygray}{gray}{0.6} 
% \definecolor{lightblue}{RGB}{235, 245, 255}
\begin{table}
\small % 减小字体大小
\centering
\resizebox{0.9\linewidth}{!}{ 
\begin{tabular}{llccccccc|c|c}
        \toprule
    	Model & Method  & TFLOPS$\downarrow$ & GenEval$\uparrow$  & Flickr30k$\uparrow$\\
        \midrule
            \multirow{3}{*}{Emu3}
            
            & \textcolor{mygray}{Base Model} &  \textcolor{mygray}{88.986}    & \textcolor{mygray}{0.423}  &  \textcolor{mygray}{5.24}\\
            & Full Computation & 88.986   &  0.460 & 17.6 \\
            \rowcolor{lightblue} 
             & \method{}  &53.489 & 0.488 & 16.2 \\
        \bottomrule
\end{tabular}
}
\caption{UniMoD for Emu3. Our method outperforms the full model in both generation and captioning tasks.}
\vspace{-20pt}

\label{tab:table_emu3}
\end{table}





==> tables/table_topk.tex <==


\begin{table}
% \begin{wraptable}{r}{0.6\textwidth} % {r}表示表格在右侧浮动，{0.5\textwidth}表示表格宽度占文本宽度的一半，可根据实际情况调整宽度值
\centering
\resizebox{1\linewidth}{!}{
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{l}{Benchmark}
&\multicolumn{1}{c}{ MME$\uparrow$ }
&\multicolumn{1}{c}{ GQA$\uparrow$ }
&\multicolumn{1}{c}{ POPE$\uparrow$ }
&\multicolumn{1}{c}{ MMMU$\uparrow$ }
&\multicolumn{1}{c}{ VQAv2{\text{(test)}}$\uparrow$ }
&\multicolumn{1}{c}{ GenEval$\uparrow$ }
\\
\midrule
Base Model
&$1032$
&$52.54$
&$77.94$ 
&$27.44$
&$62.39$ 
&$0.63$
\\
MoD
&$810$
&$46.49$
&$76.24$ 
&$26.67$
&$56.76$ 
&$0.42$
\\
MoD*
&$1005$
&$49.43$
&$77.63$ 
&$26.33$
&$59.78$ 
&$0.49$
\\
\bottomrule
\end{tabular}
}
\caption{
MoD selection in Show-o. 40\% percent of tokens are skipped at interleaved layers. MoD* denotes that capacity decreases as the layer index increases, indicating that earlier layers require more tokens for both tasks.
\label{tab:topk_selection}
\vspace{-10pt}
}
\end{table}
% \end{wraptable}





% % \begin{wraptable}{r}{0.5\textwidth} % {r}表示表格在右侧浮动，{0.5\textwidth}表示表格宽度占文本宽度的一半，可根据实际情况调整宽度值
% \begin{table}
% \centering
% \resizebox{1\linewidth}{!}{
% \setlength{\tabcolsep}{1.8pt}
% \begin{tabular}{lcccccc}
% \toprule
% \multicolumn{1}{l}{Benchmark}
% &\multicolumn{1}{c}{ MME$\uparrow$ }
% &\multicolumn{1}{c}{ GQA$\uparrow$ }
% &\multicolumn{1}{c}{ POPE$\uparrow$ }
% &\multicolumn{1}{c}{ GenEval$\uparrow$ }
% \\
% \midrule
% TopK
% &$810$
% &$46.49$
% &$76.24$ 
% &$0.42$
% \\
% TopK*
% &$1005$
% &$49.43$
% &$77.63$ 
% &$0.49$
% \\
% \bottomrule
% \end{tabular}
% }
% \caption{
% TopK selection in Show-o. 40\% percent of tokens are skipped at interleaved layers. TopK* denotes that capacity decreases as the layer index increases, indicating that earlier layers require more tokens for both tasks.
% \label{tab:topk_selection}
% }
% \end{table}
% % \end{wraptable}












==> tables/table_topk_diversity.tex <==


% \begin{wraptable}{r}{0.3\textwidth}
% \usepackage{wrapfig}
\begin{table}
\centering

\resizebox{1\linewidth}{!}{
\centering
\setlength{\tabcolsep}{1.8pt}

%
\begin{tabular}{cccccc}
% \begin{tabular}{l||ccccc||ccccc}
\toprule

% \multicolumn{1}{l|}{Benchmark}
\multicolumn{1}{c}{ MME$\uparrow$ }
&\multicolumn{1}{c}{ GQA$\uparrow$ }
&\multicolumn{1}{c}{ POPE$\uparrow$ }
&\multicolumn{1}{c}{ MMMU$\uparrow$ }
&\multicolumn{1}{c}{ VQAv2{\text{(test)}}$\uparrow$ }
&\multicolumn{1}{c}{ GenEval$\uparrow$ }

% \midrule
  % \\Value
  \\$1005$
  &$76.24$
  &$46.49$ 
  &$26.67$
  &$0.48$ 
  &$0.489$

  


  

\\ \bottomrule



\end{tabular}


}
\caption{
TopK selection on Show-o using diverse k values. 40\% tokens are skipped at the interleaved layer.
\label{tab:inference_skip_layer}
}
\vspace{-10pt}
\end{table}
% \end{wraptable}


